Dynamic Data Selection for Curriculum Learning via Ability Estimation

Curriculum learning methods typically rely on heuristics to estimate the difficulty of training examples or the ability of the model. In this work, we propose replacing difficulty heuristics with learned difficulty parameters. We also propose Dynamic Data selection for Curriculum Learning via Ability Estimation (DDaCLAE), a strategy that probes model ability at each training epoch to select the best training examples at that point. We show that models using learned difficulty and/or ability outperform heuristic-based curriculum learning models on the GLUE classification tasks.

==> tables/ddaclae_accuracies_bert-False.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Fri May 29 10:32:30 2020
\begin{table*}[ht]
\centering
\begingroup\small
\begin{tabular}{lcccccc}
  \toprule
 & MNLI & MRPC & QNLI & QQP & RTE & SST2 \\ 
  \midrule
Fully Supervised & 82.54 [$\pm$0.32] & 77.79 [$\pm$5.02] & 89.54 [$\pm$0.68] & 85 [$\pm$6.96] & 57.33 [$\pm$2.18] & 75.34 [$\pm$13.03] \\ 
  CB Linear ($d_{irt}$) & 82.57 [$\pm$0.17] & 79.71 [$\pm$3.54] & 88.36 [$\pm$1.8] & \underline{89.77} [$\pm$0.32] & \bf \underline{61.3} [$\pm$3.45] & 90.28 [$\pm$0.59] \\ 
  CB Linear ($d_{length}$) & 82.25 [$\pm$0.07] & 74.12 [$\pm$4.55] & 81.23 [$\pm$10.4] & 79.32 [$\pm$8.61] & 57.62 [$\pm$3.52] & 82.48 [$\pm$10.33] \\ 
  CB Root ($d_{irt}$) & \bf \underline{82.66} [$\pm$0.09] & \bf \underline{82.45} [$\pm$1.21] & 81.43 [$\pm$10.45] & 89.43 [$\pm$0.56] & 56.75 [$\pm$1.39] & \underline{90.37} [$\pm$0.58] \\ 
  CB Root ($d_{length}$) & 72.25 [$\pm$12.91] & 75.1 [$\pm$3.88] & \underline{89.03} [$\pm$0.59] & 76.92 [$\pm$7.77] & 52.2 [$\pm$1.72] & 82.59 [$\pm$10.05] \\ 
  DDaCLAE & 81.7 [$\pm$0.33] & 76.42 [$\pm$4.33] & \bf 89.94 [$\pm$0.24] & \bf 90.26 [$\pm$0.05] & 55.31 [$\pm$3.32] & \bf 90.83 [$\pm$0.35] \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{BERT dev set accuracy results, including 95\% confidence intervals, for each task under consideration. During training, 10\% of the training set was held out and used for early stopping. Highest overall accuracy is bolded. Highest accuracy among competence-based methods is underlined} 
\label{tab:acc_bert-False}
\end{table*}


==> tables/ddaclae_accuracies_lstm-False.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Fri May 29 09:51:41 2020
\begin{table*}[ht]
\centering
\begingroup\small
\begin{tabular}{lcccccc}
  \toprule
 & MNLI & MRPC & QNLI & QQP & RTE & SST2 \\ 
  \midrule
Fully Supervised & 64.93 [$\pm$0.29] & 69.61 [$\pm$0.31] & 62.38 [$\pm$0.81] & 80.86 [$\pm$0.09] & 50.18 [$\pm$1.42] & 84.31 [$\pm$0.54] \\ 
  CB Linear ($d_{irt}$) & 65.19 [$\pm$0.15] & \underline{70.49} [$\pm$0.19] & \underline{61.16} [$\pm$0.35] & 81.63 [$\pm$0.1] & \bf \underline{51.05} [$\pm$0.74] & 84.96 [$\pm$0.36] \\ 
  CB Linear ($d_{length}$) & 63.82 [$\pm$0.35] & 69.12 [$\pm$1.47] & 60.51 [$\pm$0.84] & 79.42 [$\pm$0.07] & 49.68 [$\pm$1.53] & 84.66 [$\pm$0.46] \\ 
  CB Root ($d_{irt}$) & \underline{65.58} [$\pm$0.13] & 70.34 [$\pm$0.39] & 61.07 [$\pm$0.55] & \bf \underline{81.86} [$\pm$0.08] & 50.36 [$\pm$0.85] & \bf \underline{85.27} [$\pm$0.24] \\ 
  CB Root ($d_{length}$) & 63.85 [$\pm$0.05] & 69.46 [$\pm$0.41] & 59.51 [$\pm$0.98] & 79.48 [$\pm$0.1] & 49.82 [$\pm$1.32] & 84.66 [$\pm$0.57] \\ 
  DDaCLAE & \bf 65.76 [$\pm$0.19] & \bf 70.75 [$\pm$0.61] & \bf 63.12 [$\pm$0.19] & 81.81 [$\pm$0.08] & 49.52 [$\pm$1.08] & 84.78 [$\pm$0.43] \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{LSTM dev set accuracy results, including 95\% confidence intervals, for each task under consideration. During training, 10\% of the training set was held out and used for early stopping. Highest overall accuracy is bolded. Highest accuracy among competence-based methods is underlined} 
\label{tab:acc_lstm-False}
\end{table*}


==> tables/ddaclae_avgEpoch_bert-False.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Fri May 29 10:32:30 2020
\begin{table*}[ht]
\centering
\begingroup\small
\begin{tabular}{lcccccc}
  \hline
ExpName & MNLI & MRPC & QNLI & QQP & RTE & SST2 \\ 
  \hline
Fully Supervised & \bf 1.8 [$\pm$0.26] & 4.6 [$\pm$2.09] & \bf 2 [$\pm$0.41] & \bf 3.4 [$\pm$0.89] & 5.6 [$\pm$1.68] & \bf 2.6 [$\pm$0.89] \\ 
  CB Linear ($d_{irt}$) & 6.6 [$\pm$0.32] & 7.4 [$\pm$1.28] & 6 [$\pm$0.41] & 8.2 [$\pm$0.26] & 7.6 [$\pm$1.88] & 8 [$\pm$0.58] \\ 
  CB Linear ($d_{length}$) & 6.4 [$\pm$0.32] & 3.6 [$\pm$2.17] & 6.2 [$\pm$1.67] & 5.8 [$\pm$2.59] & 7.8 [$\pm$0.49] & 6.8 [$\pm$1.62] \\ 
  CB Root ($d_{irt}$) & 6 [$\pm$0] & 7.8 [$\pm$0.76] & 6 [$\pm$0.58] & 7.2 [$\pm$0.76] & \bf 5.4 [$\pm$2.13] & 7.6 [$\pm$0.67] \\ 
  CB Root ($d_{length}$) & 5 [$\pm$1.09] & \bf 4 [$\pm$1.94] & 4.6 [$\pm$0.78] & \bf 3.4 [$\pm$1.68] & 7.4 [$\pm$2.17] & 7.6 [$\pm$0.78] \\ 
  DDaCLAE & 8.4 [$\pm$1.52] & 5.2 [$\pm$2.35] & 2.4 [$\pm$0.32] & 7.2 [$\pm$1.27] & \bf 5.4 [$\pm$1.88] & 7 [$\pm$0.58] \\ 
   \hline
\end{tabular}
\endgroup
\caption{Average number of training epochs until convergence for each model, with 95\% confidence intervals.} 
\label{tab:epoch_bert-False}
\end{table*}


==> tables/ddaclae_avgEpoch_lstm-False.tex <==
% latex table generated in R 3.6.2 by xtable 1.8-4 package
% Fri May 29 09:51:41 2020
\begin{table*}[ht]
\centering
\begingroup\small
\begin{tabular}{lcccccc}
  \hline
ExpName & MNLI & MRPC & QNLI & QQP & RTE & SST2 \\ 
  \hline
Fully Supervised & \bf 18 [$\pm$1.13] & \bf 17.67 [$\pm$0.88] & 34.67 [$\pm$15.44] & 71.17 [$\pm$9.9] & 64.67 [$\pm$6.28] & 50.17 [$\pm$10.44] \\ 
  CB Linear ($d_{irt}$) & 39.92 [$\pm$0.84] & 44.42 [$\pm$1.83] & 51.67 [$\pm$8.17] & 76.58 [$\pm$5.89] & 76.5 [$\pm$6.81] & 74.25 [$\pm$2] \\ 
  CB Linear ($d_{length}$) & 37.6 [$\pm$1.68] & 56.2 [$\pm$10.28] & 57.4 [$\pm$21.36] & 92 [$\pm$4.47] & 68.8 [$\pm$17.07] & 78.6 [$\pm$7.49] \\ 
  CB Root ($d_{irt}$) & 31 [$\pm$0.47] & 32.17 [$\pm$1.64] & 50.25 [$\pm$10.75] & 79.17 [$\pm$6.47] & 55.42 [$\pm$6.34] & 73.83 [$\pm$3.35] \\ 
  CB Root ($d_{length}$) & 31 [$\pm$1.85] & \bf 34.2 [$\pm$9.12] & 81.8 [$\pm$16.33] & 83.6 [$\pm$10.12] & 34.2 [$\pm$15.42] & 59.6 [$\pm$6.33] \\ 
  DDaCLAE & 22.17 [$\pm$0.86] & 36.83 [$\pm$11.25] & \bf 23.5 [$\pm$1.86] & \bf 70 [$\pm$14.72] & 36.67 [$\pm$7.99] & \bf 50 [$\pm$7.55] \\ 
   \hline
\end{tabular}
\endgroup
\caption{Average number of training epochs until convergence for each model, with 95\% confidence intervals.} 
\label{tab:epoch_lstm-False}
\end{table*}

